Maximal analytic extensions of the Emparan-Reall black ring

We construct a Kruskal-Szekeres-type analytic extension of the Emparan-Reall black ring, and investigate its geometry. We prove that the extension is maximal, globally hyperbolic, and unique within a natural class of extensions. The key to those results is the proof that causal geodesics are either complete, or approach a singular boundary in finite affine time. Alternative maximal analytic extensions are also constructed.

==> bhmacros.tex <==
\newcommand{\zk}{{\mathring k}}



\newcommand{\Spn}{S^+_0}
\newcommand{\Spz}{S^+_0}
\newcommand{\mcEp}{{\mcE^+}}
\newcommand{\mcEpz}{{\mcE^+_0}}
\newcommand{\mcEm}{{\mcE^-}}
\newcommand{\mcEmz}{{\mcE^-_0}}

\newcommand{\ii}{{\mathrm{i}}}

\newcommand{\jlcasug}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca suggests!}
}}{\color{blue}{#1}}\color{black}\ }

\newcommand{\hfourg}{\hat \fourg}

\newcommand{\oft}{{outer future trapped}}
\newcommand{\wpt}{{weakly past trapped}}

\newcommand{\kk}[1]{}%{\mnote{{\bf If we consider the KK case:} #1}}

\newcommand{\mexp}{\mbox{\rm exp}}

\newcommand{\zR}{\mathring R}
\newcommand{\zD}{\mathring D}
\newcommand{\zA}{\mathring A}
\newcommand{\mzh}{\mathring h}


\newcommand{\hypwithhat}{\hathyp}
\newcommand{\hathyp}{\,\,\widehat{\!\!\hyp}}

\newcommand{\Span}{\mathrm{Span}}

\newcommand{\odoc}{\overline{\doc}}
\newcommand{\ohyp}{\,\,\overline{\!\!\hyp}}
\newcommand{\pohyp}{\partial\ohyp}

\newcommand{\aregular}{{an {\regular}}}
\newcommand{\regular}{$I^+$--regular}%\newchange{terminology changed (macro, can be restored by resetting to ``regular")}}

\newcommand{\hthreeg}{h}


\newcommand{\doce}{\doc_\epsilon}

\newcommand{\odocIp}{\overline{\doc}\cap I^+(\Mext)}
\newcommand{\odocup}{{\doc}\cup \mcH_0^+}
\newcommand{\llambda}{\lambda}

\newcommand{\ue}{u_{\epsilon}}
\newcommand{\uee}{u_{\epsilon,\eta}}

\newcommand{\bmcM}{\,\,\,\,\widetilde{\!\!\!\!\mcM}}
\newcommand{\bfourg}{\widetilde{\fourg}}

\newcommand{\eean}{\nonumber\end{eqnarray}}

\newcommand{\lp}{\ell}

\newcommand{\tSp}{\tilde S_p}
\newcommand{\Sp}{S_p}

\newcommand{\dgtcp}{\dgt}%{(\dgt\cup \zh)}
\newcommand{\dgtc}{\dgt}%{\dgt\cup \zh}

\newcommand{\id}{{\rm id}}

\newcommand{\Zd}{{\mcZ}_{\dgt}}


\newcommand{\mcHp}{{\mcH^+}}
\newcommand{\mcHpz}{{\mcH^+_0}}
\newcommand{\mcHm}{{\mcH^-}}
\newcommand{\mcHmz}{{\mcH^-_0}}

\newcommand{\zN}{\mathring N}

\newcommand{\mcY}{{\mycal Y}}
\newcommand{\mcX}{{\mycal X}}


\newcommand{\Nndg}{N_{\mbox{\scriptsize\rm  ndh}}}
\newcommand{\Ndg}{N_{\mbox{\scriptsize\rm  dh}}}
\newcommand{\Nndh}{N_{\mbox{\scriptsize\rm  ndh}}}
\newcommand{\Ndh}{N_{\mbox{\scriptsize\rm  dh}}}
\newcommand{\Naf}{N_{\mbox{\scriptsize\rm  AF}}}
\newcommand{\alpharate}{\lambda}
\newcommand{\zalpha}{\mathring \alpha}

\newcommand{\puncti}{a_i}
\newcommand{\ai}{\puncti}


\newcommand{\mcS}{{\mycal S}}


\newcommand{\nic}{}
\newcommand{\phypa}{\partial\mcS_{(a)} }
\newcommand{\Ya}{{}^{(a)}Y }
\newcommand{\Ja}{{}^{(a)}J }
\newcommand{\Oma}{{}^{(a)}\Omega }
\newcommand{\Xa}{{}^{(a)}X }
\newcommand{\Sa}{{}^{(a)}S }
\newcommand{\Qea}{{}^{(a)}Q^E}
\newcommand{\Qba}{{}^{(a)}Q^B}
\newcommand{\phiea}{{}^{(a)}\Phi^E}
\newcommand{\phiba}{{}^{(a)}\Phi^B}
\newcommand{\mcHa}{{}^{(a)}\mcH}

\newcommand{\hypo}{\,\,\mathring{\!\! \hyp}}
\newcommand{\ohypo}{\overline{\hypo}}

\newcommand{\Kz}{K_\kl 0}

\newcommand{\fourge}{\fourg_\epsilon}

\newcommand{\Cp}{ \mcC^+ }
\newcommand{\Cpe}{ \mcC^+ _\epsilon}
\newcommand{\Ct}{ \mcC^+_t}
\newcommand{\Ctm}{ \mcC^+_{t_-}}
\newcommand{\hStmR}{\hat S_{t_-,R}}
\newcommand{\hStR}{\hat S_{t,R}}
\newcommand{\hSzR}{\hat S_{0,R}}
\newcommand{\hSts}{\hat S_{\tau,\sigma}}

\newcommand{\Sone}{\Sz}
\newcommand{\Sonep}{\Sz}%{S_{0,p}}
\newcommand{\Soneq}{S_{0,q}}
\newcommand{\Stp}{S_{t,p}}
\newcommand{\Stq}{S_{t,q}}
\newcommand{\Sz}{S_0}

\newcommand{\bw}{\bar w}
\newcommand{\bzeta}{\bar \zeta}

\newcommand{\zMtwo}{\mathring{M}{}^2}
\newcommand{\Mtwo}{{M}{}^2}
\newcommand{\bMtwo}{{\bar M}{}^2}
\newcommand{\hMtwo}{{\hat M}{}^2}

\newcommand{\hypext}{\hyp_{\mbox{\scriptsize \rm ext}}}
\newcommand{\Mtext}{\Sext}%{M_{\mbox{\scriptsize \rm ext}}}
\newcommand{\Mint}{\mcM_{\mbox{\scriptsize \rm int}}}
\newcommand{\mcMext}{\Mext}

\newcommand{\mcHN}{\mcN}
\newcommand{\mcNH}{\mcH}

\newcommand{\hS }{{\hat S }}
\newcommand{\hSq}{{\hat S_q}}
\newcommand{\hSp}{{\hat S_p}}
\newcommand{\hSpn}{{\hat S_{p_n}}}
\newcommand{\hSqn}{{\hat S_{q_n}}}
\newcommand{\mcA}{\mycal A}
\newcommand{\mcZ}{\mycal Z}

\newcommand{\zh}{{\,\,\widetilde{\!\!\mcZ}}}
\newcommand{\dgt}{{\mycal Z}_{dgt}}

\newcommand{\kl}[1]{{(#1)}}

\newcommand{\Uone}{{\mathrm{U(1)}}}






 % The next ones are HR
\newcommand{\Sm}{\ensuremath{\Sigma_{-}}}
\newcommand{\Nt}{\ensuremath{N_{2}}}
\newcommand{\Nth}{\ensuremath{N_{3}}}



\newcommand{\jlca}[1]{\mnote{{\bf jlca:} #1}}






\newcommand{\jlcared}[1]{{\color{red}\mnote{{\color{red}{\bf jlca:}
#1} }}}
\newcommand{\jlcachange}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca:}
changed on 18.IX.07}}{\color{blue}{#1}}\color{black}\ }

\newcommand{\jlcachangeb}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca:}
changed on 19.IX.07}}{\color{blue}{#1}}\color{black}\ }
\newcommand{\jlcachangec}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca:}
changed on 20.IX.07}}{\color{blue}{#1}}\color{black}\ }
\newcommand{\jlcachanged}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca:}
changed after 9.X.07}}{\color{blue}{#1}}\color{black}\ }
\newcommand{\jlcachangeXIII}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca:}
changed after 13.X.07}}{\color{blue}{#1}}\color{black}\ }


\newcommand{\jlcaadded}[1]{{\color{blue}\mnote{\color{blue}{\bf jlca:}
added on 20.IX.07}}{\color{blue}{#1}}\color{black}\ }
\newcommand{\sse }{\Longleftrightarrow}
\newcommand{\se}{\Rightarrow}
\newcommand{\uu}{{\bf u}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbH}{\mathbb{H}}

\newcommand{\cof}{\operatorname{cof}}
\newcommand{\dive}{\operatorname{div}}
\newcommand{\curl}{\operatorname{curl}}
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\rank}{\operatorname{rank}}
\def\G{{\mycal G}}
\def\scro{{\mycal O}}
\def\Doc{\doc}%{{\mycal Doc}}
\def\scrip{\scri^{+}}%
\def\scrp{{\mycal I}^{+}}%
\def\Scri{\scri}
\def\scra{{\mycal A}}
\def\Scra{\cup_{i}\scra_i}
\def\scru{{\mycal U}}
\def\scrw{{\mycal W}}
\def\scrv{{\mycal V}}
\def\scrs{{\mycal S}}
%\def\ext{{\mycal S}_{ext}}
%\def\Mext{ M_{ext}}
%\def\int{{\mycal S}_{int}}
%\def\doc{{\mycal Doc}}
\def\rot{{\mycal R}}
\def\khor{{\mycal H}}
%\def\Lie{{\mycal L}}
\def\e{\wedge}
\def\d{\partial}
\def\KK{\phi^K}
\def\K0{\phi^{K_0}}
%\def\X{\phi^{X}}
\def\Kdot{\phi^{K}\cdot}
\def\X.{\phi^{X}\cdot}
\def\normK{W}%{|K_0\e...\e K_{D-3}|^2}

\newcommand{\hyphat}{\,\,\,\widehat{\!\!\!\hyp}}
\newcommand{\hmcM}{\,\,\,\widehat{\!\!\!\mcM}}







\newcommand{\newF}{\lambda}


%\newcommand{\Ric}{\operatorname{Ric}}
\newcommand{\Int}{\operatorname{Int}}
\newcommand{\Tr}{\operatorname{Tr}}


\newcommand{\myuu}{u}

\newcommand{\oX}{\overline X}
\newcommand{\oY}{\overline Y}
\newcommand{\op}{\overline p}
\newcommand{\oq}{\overline q}



\newcommand{\hg}{{\hat g}}
\newcommand{\mcEh}{{{\mycal E}^+_\hyp}}

{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{equation}{section}
\renewcommand{\theequation}{\thesection.\arabic{equation}}
{\catcode `\@=11 \global\let\AddToReset=\@addtoreset}
\AddToReset{figure}{section}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}


\newcommand{\ptcKcite}[1]{.\cite{#1}}

\newcommand{\fourg}{{\mathfrak g }}

\newcommand{\refcite}[1]{\cite{#1}}
\newcommand{\levoca}[1]{\ptc{#1}}


\newcommand{\umac}{\gamma}%
\newcommand{\metrict}{\threeg }%


\newcommand{\mcN}{{\mycal N}}
\newcommand{\mcNX}{{\mycal N(X)}}

\newcommand{\cf}{cf.,}


\newcommand{\gcirc}{{\mathring{g}}_{ab}}
\let\a=\alpha\let\b=\beta \let\g=\gamma \let\d=\delta\let\lb=\lambda
\newcommand{\sts}{spacetimes}
\newcommand{\calM}{{\mcM}}
\newcommand{\calH}{{\mcH}}
\newcommand{\el}{e^{2\lb}}
\newcommand{\hysf}{hypersurface}
%\newcommand{\cH}{{\mycal  H}}
\newcommand{\OOmega}{\omega}

\newcommand{\nopcite}[1]{}

\newcommand{\hypM}{\hyp}

\newcommand{\gschw}{h_{\mbox{\scriptsize \rm Schw}}}
\newcommand{\gsch}{\gschw}

\newcommand{\calSJr}{{\mycal  S}_{(J_0,\rho_0)}}
\newcommand{\Ima}{\mbox{\rm Im}}
\newcommand{\Ker}{\mbox{\rm Ker}}
\newcommand{\sgstatic}{{strictly globally static{}}}
\newcommand{\gstatic}{{globally static{}}}
\newcommand{\riemg}{g}
\newcommand{\riemgz}{g_0}
\newcommand{\hhat}{\ghat}
\newcommand{\DeltaL}{\Delta_{\mathrm L}}
\newcommand{\ghat}{\gamma}%{{\widehat \riemg}}
\newcommand{\hzhat}{\gamma_0}%{{\widehat \riemgz}}
\newcommand{\holder}{H\"older }
%\newcommand{\<}{\langle}
%\renewcommand{\>}{\rangle}
\newcommand{\del}{\partial}
\newcommand{\Mbar}{{\overline M}}
\newcommand{\gbar}{{\overline \riemg}}
%\renewcommand{\hbar}{{\overline \riemgz}}
\newcommand{\dm}{{\partial M}}
\newcommand{\dminfty}{{\partial_\infty M}}
\newcommand{\dmo}{{\partial_0 M}}
%\newcommand{\letters}
% {\renewcommand{\theenumi}{\alph{enumi}}
%   \renewcommand{\labelenumi}{(\theenumi)}}
%\newcommand{\romanletters}
  {\renewcommand{\theenumi}{\roman{enumi}}
   \renewcommand{\labelenumi}{(\theenumi)}}








\newcommand{\bS}{{\overline \Sigma}}
\newcommand{\pS}{{\partial \Sigma}}
\newcommand{\tp}{\tau_p}
\newcommand{\hF}{\hat F}
\newcommand{\signX}{\mathrm{sign}X}
\newcommand{\mnu}{\nu}
\newcommand{\homega}{{\widehat{\Omega}}}%
\newcommand{\kerp}{\mathrm{Ker}_p\nabla X}%
\newcommand{\kerpi}{\mathrm{Inv}_p}%
\newcommand{\const}{\mathrm{const}}
\newcommand{\ml}{{M_{0,n-2\ell}}}
\newcommand{\mil}{{M_{\mathrm{iso},\ell}}}
\newcommand{\mtwo}{{M_{0,n-2}}}
\newcommand{\mfour}{{M_{0,n-4}}}
\newcommand{\sell}{\pi_\Sigma(\ml)}
\newcommand{\sfour}{\pi_\Sigma(\mfour)}
\newcommand{\stwo}{\pi_\Sigma(\mtwo)}
\newcommand{\mi}{{M_{0,n-2i}}}
\newcommand{\mj}{{M_{0,n-2j}}}
\newcommand{\htau}{{\hat \tau}}
\newcommand{\ttau}{{\tilde \tau}}
\newcommand{\zM}{{\mathring{M}}}
\newcommand{\ztau}{{\mathring{\tau}}}
\newcommand{\zSigma}{{\mathring{\Sigma}}}
\newcommand{\sings}{{\Sigma_{\mathrm{sing,iso}}}}
\newcommand{\miso}{{M_{\mathrm{iso}}}}
\newcommand{\psings}{{\partial\Sigma_{\mathrm{sing,iso}}}}
\newcommand{\sing}{{\Sigma_{\mathrm{sing}}}}
\newcommand{\singt}{{\Sigma_{\mathrm{sing},0}}}
\newcommand{\psingt}{{\partial\Sigma_{\mathrm{sing},0}}}
\newcommand{\Ein}{\operatorname{Ein}}
\newcommand{\hlambda}{\hat \lambda}
\newcommand{\mLX}{{\mcL_X}}
\newcommand{\mcE}{{\mycal E}}
\newcommand{\mcC}{{\mycal C}}
\newcommand{\mcD}{{\mycal D}}
\newcommand{\mcW}{{\mycal W}}
\newcommand{\lormet  }{{\frak g}}
\newcommand{\ApSwSw}{Appendix~\ref{SwSs}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\M}{\EuScript M}
\newcommand{\Lie}{\EuScript L}
\newcommand{\nablash}{\nabla{\kern -.75 em
     \raise 1.5 true pt\hbox{{\bf/}}}\kern +.1 em}
\newcommand{\Deltash}{\Delta{\kern -.69 em
     \raise .2 true pt\hbox{{\bf/}}}\kern +.1 em}
\newcommand{\Rslash}{R{\kern -.60 em
     \raise 1.5 true pt\hbox{{\bf/}}}\kern +.1 em}
\newcommand{\Div}{\operatorname{div}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\Rfour}{\bar R}

\newcommand{\tthreeg}{\tilde\threeg}
\newcommand{\tcalD}{\widetilde\calD}
\newcommand{\tnabla}{\tilde \nabla}

\newcommand{\tD}{\tilde D}

\newcommand{\gammab}{\bar\gamma}
\newcommand{\chib}{\bar\chi}
\newcommand{\gb}{\bar g}
\newcommand{\Nb}{\bar N}
\newcommand{\Hb}{\bar H}
\newcommand{\Ab}{\bar A}
\newcommand{\Bb}{\bar B}
\newcommand{\betah}{{\hat\beta}}
\newcommand{\chit}{\tilde\chi}
%\newcommand{\Nt}{\tilde N}
\newcommand{\Ht}{\tilde H}
%\newcommand{\Sphere}{\mathbb S}
\newcommand{\Ric}{\operatorname{Ric}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\st}{\colon\>}







\newcommand{\hbound}{\mathring{\mathsf{H}}}
\newcommand{\cbord}{{\mathsf{C}}}
\newcommand{\pM}{\partial M}
\newcommand{\hM}{\widehat{M}}
\newcommand{\chyp}{\mathcal C}
\newcommand{\hhyp}{\mathring{\mathcal H}}
\newcommand{\bnabla}{\overline{\nabla}}
\newcommand{\maclK}{{\mathcal K}}
\newcommand{\maclKzo}{{\mathcal K}^{\bot_g}_0}
\newcommand{\maclKz}{{\mathcal K}_0}
\newcommand{\hbord}{\hbound}%
\newcommand{\cKi}{{\mycal K}_{i0}}
%\newcommand{\fourg}{{}^{4}g}
\newcommand{\mcO}{{\mycal O}}
\newcommand{\mcT}{{\mycal T}}
\newcommand{\mcU}{{\mycal U}}
\newcommand{\mcV}{{\mycal V}}
\newcommand{\eug}{{\frak G}}






\newcommand{\rd}{\,{ d}} % exterior differential






\newcommand{\ourU}{\mathbb U}
\newcommand{\ourW}{\mathbb W}
\newcommand{\hyp}{{\mycal S}}%{\Sigma}{{\mycal S}}

\newcommand{\bhyp}{\overline{\hyp}}%{\,\,\,\overline{\!\!\!\mycal S}}






\newcommand{\bg}{{\overline{g}_\Sigma}}






\newcommand{\Bgamma}{{B}} % koneksja tla
\newcommand{\bmetric}{{b}} % metryka tla






\newcommand{\Kp}{{\mathfrak g}} %{\pi}} % kontrawariantna gestosc metryki
                            %na czasoprzestrzeni
\newcommand{\KA}{p} % ped sprzezony do kontrawariantnej gestosci
                    % metryki (A duze w innych pracach JK i JJ)
%\newcommand{\E}[1]{{\rm e}^{#1}}
%\newcommand{\kolo}[1]{\stackrel{\circ}{#1}}
%\newcommand{\ve}{\varepsilon}
\newcommand{\gthreeup}{\,{}^3g} %three dimensional metric in
                                %space--time, used for the inverse
\newcommand{\cO}{{\mathscr O}}
\newcommand{\arcsh}{{\rm argsh}}

\newcommand{\threeg}{\gamma}

\newcommand{\detthreeg}{{\det(\threeg_{ij})}} % determinant of the
                                             % three dimensional
                                             % metric pulled back
                               %to the model space
\newcommand{\lapse}{{\nu}} % the lapse function on the model space
\newcommand{\shift}{{\beta}} % the shift vector field on the model
                             % space
\newcommand{\threeP}{{\pi}} %three dimensional ADM momentum pulled back
                               %to the model space
\newcommand{\tildetg}{{\tilde \threeg}} % conformally rescaled metric
\newcommand{\hst}{{\breve{h}}} % standard round metric on the two
                              % sphere





\newcommand{\zn} {\mathring{\nabla}} % pochodna metryki tla
\newcommand{\znabla} {\mathring{\nabla}} % pochodna metryki tla
\newcommand{\mn} {M} %{{}^{n-1}M} %the n-1 dimensional manifold



\newcommand{\eg}{e.g.,}


\newcommand{\can}{{\mathrm \scriptsize can}}

\newcommand{\mcM}{{\mycal M}}
\newcommand{\mcR}{{\mycal R}}
\newcommand{\mcH}{{\mycal H}}
\newcommand{\mcK}{{\mycal K}}
\newcommand{\notreP}{{\widehat P}}
\newcommand{\ninfty}{N_\infty}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\bean}{\begin{eqnarray}\nonumber}
\newcommand{\kidap}{KID-hole}
\newcommand{\kidhor}{KID-horizon}
\newcommand{\kidaps}{KID-holes}
\newcommand{\bel}[1]{\begin{equation}\label{#1}}
\newcommand{\beal}[1]{\begin{eqnarray}\label{#1}}
\newcommand{\beadl}[1]{\begin{deqarr}\label{#1}}
\newcommand{\eeadl}[1]{\arrlabel{#1}\end{deqarr}}
\newcommand{\eeal}[1]{\label{#1}\end{eqnarray}}
\newcommand{\eead}[1]{\end{deqarr}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\eeaa}{\end{eqnarray*}}
\newcommand{\nn}{\nonumber}
\newcommand{\Hess}{\mathrm{Hess}\,}
\newcommand{\Ricc}{\mathrm{Ric}\,}
\newcommand{\Riccg}{\Ricc(g)}
\newcommand{\Lpsi}{L^{2}_{\psi}}
\newcommand{\Lpsione}{\zH1_{\phi,\psi}}
\newcommand{\Lpsitwo}{\zH^{2}_{\phi,\psi}}







\newcommand{\Lpsig}{L^{2}_{\psi}(g)}
\newcommand{\Lpsioneg}{\zH1_{\phi,\psi}(g)}
\newcommand{\Lpsitwog}{\zH^{2}_{\phi,\psi}(g)}
\newcommand{\Lpsikg}[2]{\zH^{#1}_{\phi,\psi}(#2)}


\newcommand{\zg}{\mathring{g}}




\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\divr }{\mbox{\rm div}\,}
\newcommand{\tr}{\mbox{\rm tr}\,}
\newcommand{\ext}{{\mathrm{ext}}}%{\mbox{\rm \scriptsize ext}\,}
\newcommand{\J}{\delta J}
\newcommand{\source}{\delta \rho}
\newcommand{\eq}[1]{\eqref{#1}}
%\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\Eq}[1]{Equation~(\ref{#1})}
\newcommand{\Eqsone}[1]{Equations~(\ref{#1})}
\newcommand{\Eqs}[2]{Equations~(\ref{#1})-\eq{#2}}
\newcommand{\Sect}[1]{Section~\ref{#1}}
\newcommand{\Lem}[1]{Lemma~\ref{#1}}
%\newcommand{\D}[1]{Definition~\ref{#1}}












\newcommand{\zmcH }{\,\,\,\,\mathring{\!\!\!\!\mycal H}{}}








%
%\renewcommand{\theequation}{\thesection.\arabic{equation}}
%
%\let\ssection=\section
%
%\renewcommand{\section}{\setcounter{equation}{0}\ssection}
%
%
\newtheorem{defi}{\sc Coco\rm}[section]
\newtheorem{theorem}[defi]{\sc Theorem\rm}
\newtheorem{Theorem}[defi]{\sc Theorem\rm}
\newtheorem{Disc}[defi]{\sc Discussion\rm}
\newtheorem{Conjecture}[defi]{\sc Conjecture\rm}
\newtheorem{Stat}[defi]{}
\newtheorem{lemma}[defi]{Lemma}
%\theoremstyle{plain}
\newtheorem{prop}[defi]{\sc Proposition\!\rm}
\newtheorem{Definition}[defi]{\sc Definition\rm}
\newtheorem{Def}[defi]{\sc Definition\rm}
\newtheorem{theor}[defi]{\sc Theorem\rm}
\newtheorem{Proposition}[defi]{\sc Proposition\rm}
\newtheorem{proposition}[defi]{\sc Proposition\rm}
\newtheorem{lem}[defi]{\sc Lemma\!\rm}
\newtheorem{Lems}[defi]{\sc Lemma\!\rm}
\newtheorem{Lemma}[defi]{\sc Lemma\!\rm}
%\newtheorem{cor}[defi]{\sc Corollary\!\rm}%
\newtheorem{cor}[defi]{\sc Corollary\!\rm}
\newtheorem{Corollary}[defi]{\sc Corollary\!\rm}


\theoremstyle{remark} \theorembodyfont{\upshape}
\newtheorem{Example}[defi]{{\sc Example}\rm}
\newtheorem{Remark}[defi]{{\sc Remark}\rm}
\newtheorem{Remarks}[defi]{{\sc Remarks}\rm}
%\newtheorem{example}[defi]{{\sc Example}\rm}
%\newtheorem{remark}[defi]{{\sc Remark}\rm}
\newtheorem{examp}[defi]{{\sc Example}\rm}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%\newcommand{\proof}{\noindent {\sc Proof:\ }}

\def \Reel{\mathbb{R}}
\def \C{\mathbb{C}}
\def \R {\Reel}
\def \Hyp{\mathbb{H}}
\newcommand{\mcL}{{\mycal L}}
\def \Nat{\mathbb{N}}
\def \Z{\mathbb{Z}}
\def \N {\Nat}
\def \Sphere{\mathbb{S}}
%\newcommand{\T}{\Bbb{T}}






%\newcommand{\Reel}[0]{\mbox{$\mathbb{R} $}}






%\newcommand{\Hyp}[0]{\mbox{$\mathbb{H} $}}






%\newcommand{\Nat}[0]{\mbox{$\mathbb{N} $}}






%\newcommand{\Sphere}[0]{\mbox{$\mathbb{S} $}}






%\newcommand{\Reel}[0]{\mbox{$\mathit{R} $}}






%\newcommand{\Hyp}[0]{\mbox{$\mathit{H} $}}






%\newcommand{\Nat}[0]{\mbox{$\mathit{N} $}}






%\newcommand{\Sphere}[0]{\mbox{$\mathit{S} $}}






\newcommand{\bM}{\,\overline{\!M}}






\newcommand{\zHkpp}{\zHk_{\phi,\psi}}
\newcommand{\Hkpp}{H^k_{\phi,\psi}}
\newcommand{\zHk}{\zH^k}
\newcommand{\zH}{\mathring{H}}









%%%%%%%%%%%%%%%%%%%%%%% notes en marge numerotees %%%%%%%%%%%%%%%%%%%






\newcounter{mnotecount}[section]






\renewcommand{\themnotecount}{\thesection.\arabic{mnotecount}}




\newcommand{\mnote}[1]%{}
{\protect{\stepcounter{mnotecount}}$^{\mbox{\footnotesize $%
\!\!\!\!\!\!\,\bullet$\themnotecount}}$ \marginpar{%\color{red}
\raggedright\tiny\em $\!\!\!\!\!\!\,\bullet$\themnotecount: #1} }

\newcommand{\ednote}[1]{}%{\mnote{#1}}

\newcommand{\mcmg}{$(\mcM,\fourg)$}


 % The next ones are HR%
%\newcommand{\Sm}{\ensuremath{\Sigma_{-}}}
%\newcommand{\No}{\ensuremath{N_{1}}}
%\newcommand{\Nt}{\ensuremath{N_{2}}}
%\newcommand{\Nth}{\ensuremath{N_{3}}}




\newcommand{\cem}[1]{\textcolor{bluem}{\emph{ #1}}}
\newcommand{\cbf}[1]{\textcolor{bluem}{\bf #1}}
\newcommand{\rbf}[1]{\textcolor{red}{\bf #1}}

%\definecolor{turquoise}{rgb}{0.25,0.8,0.7}
\definecolor{bluem}{rgb}{0,0,0.5}



%Il existe deux repères pour cela :
%+ cyan, magent, yellow, black
\definecolor{mycolor}{cmyk}{0.5,0.1,0.5,0}
\definecolor{michel}{rgb}{0.5,0.9,0.9}
%\newcmykcolor{le_nom_de_la_couleur}{w x y z}
%avec w,x,y,z entre 0.0 et 1.0

%+ red,green, blue et la commande :
\definecolor{turquoise}{rgb}{0.25,0.8,0.7}
\definecolor{bluem}{rgb}{0,0,0.5}



\definecolor{MDB}{rgb}{0,0.08,0.45}
\definecolor{MyDarkBlue}{rgb}{0,0.08,0.45}


\definecolor{MLM}{cmyk}{0.1,0.8,0,0.1}
\definecolor{MyLightMagenta}{cmyk}{0.1,0.8,0,0.1}

\definecolor{HP}{rgb}{1,0.09,0.58}

\newcommand{\opp}{\mnote{{\color{HP} open problem}}}

\newcommand{\jc}[1]{\mnote{{\bf jc:} #1}}
\newcommand{\ptc}[1]{\mnote{{\bf ptc:} #1}}
\newcommand{\newchange}[1]{\mnote{{\bf ptc, new change after 29 III 08:} #1}}

\newcommand{\LA} {\bf LA:}
\newcommand{\ptca}[1]{{\color{red}\mnote{{\color{black}{\bf ptc, 8.VIII.07:}
#1} }}}
\newcommand{\ptcb}[1]{{\color{red}\mnote{{\color{red}{\bf ptc, 9.VIII.07:}
#1} }}}
\newcommand{\ptcc}[1]{{\color{red}\mnote{{\color{red}{\bf ptc, 10.VIII.07:}
#1} }}}
\newcommand{\ptcd}[1]{{\color{red}\mnote{{\color{red}{\bf ptc, after 4XI07:}
#1} }}}
\newcommand{\ptce}[1]{{\color{red}\mnote{{\color{red}{\bf ptc, after 4XI07:}
#1} }}}


\newcommand{\changea}[1]{{\color{MLM}\mnote{\color{black}{\bf ptc:}
changed on 8.VIII.07}}{\color{black}{#1}}\color{black}\ }
\newcommand{\changeb}[1]{{\color{MLM}\mnote{\color{MLM}{\bf ptc:}
changed}}{\color{MLM}{#1}}\color{black}\ }
\newcommand{\changec}[1]{{\color{red}\mnote{\color{MLM}{\bf ptc:}
changed on 10.VIII.07}}{\color{MLM}{#1}}\color{black}\ }


\newcommand{\changed}[1]{{ \mnote{ {\bf ptc:}
changed}}{\sc {#1}} \ }
%
%\newcommand{\added}[1]{{\color{black}\mnote{\color{MDB}{\bf ptc:} added
%}}{\color{black}{#1}}\color{black}\ }
\newcommand{\added}[1]{{ \mnote{ {\bf ptc:} added
}}{\sc{#1}} \ }

\newcommand{\adda}[1]{{\color{MDB}\mnote{\color{MDB}{\bf ptc:} added
who knows when} {\color{MDB}{#1}}}\color{black}\ }
\newcommand{\addc}[1]{{\color{MDB}\mnote{\color{MDB}{\bf ptc:} added
on 10.VIII.07}}{\color{MDB}{#1}}\color{black}\ }
\newcommand{\addd}[1]{{\color{MDB}\mnote{\color{MDB}{\bf ptc:} added
after 4XI07}}{\color{MDB}{#1}}\color{black}\ }

\newcommand{\reworda}[1]{{\color{green}\mnote{\color{green}{\bf ptc:}
reworded on 8.VIII.07}}{\color{green}{#1}}\color{black}\ }





\newcommand{\mcMX}{\mcM_X}

\newcommand{\pdoc}{\partial \doc}
\newcommand{\loc}{{\textrm{loc}}}


\newcommand{\xflat}{X^\flat}
\newcommand{\kflat}{K^\flat}
\newcommand{\yflat}{Y^\flat}
\newcommand{\Sext}{\hyp_{\mathrm{ext}}}
\newcommand{\Mext}{\mcM_{\mathrm{ext}}}
\newcommand{\Mextl}{\Mext^\lambda}
\newcommand{\Mextls}{\Mext^{\lambda_*}}
\newcommand{\doc}{\langle\langle \mcMext\rangle\rangle}
\newcommand{\docl}{\langle\langle\mcMext^\lambda\rangle\rangle}
\newcommand{\docls}{\langle\langle \mcMext^{\lambda_*}\rangle\rangle}
\newcommand{\doclo}{\langle\langle \mcMext^{\lambda_1}\rangle\rangle}
\newcommand{\doclt}{\langle\langle \mcMext^{\lambda_2}\rangle\rangle}
\newcommand{\Tau}{\tau}

\newcommand{\bcM}{{\,\,\,\overline{\!\!\!\mcM}}}%{\,\,\,\,\widetilde{\!\!\!\!\cM}}
\newcommand{\tcM}{\,\,\,\,\widetilde{\!\!\!\!\cM}}
%\newcommand{\tg}{{\tilde g}}
\newcommand{\hJ}{{\hat J}}
\newcommand{\sthd}{{}^{\star_g}}
\newcommand{\hG}{\widehat \Gamma}
\newcommand{\hD}{\widehat D}
\newcommand{\hxi}{\hat \xi}
\newcommand{\hxib}{\hat{\xib}}
\newcommand{\heta}{\hat \eta}
\newcommand{\hetab}{\hat{\etab}}
\newcommand{\home}{\hat{\omega}}
\newcommand{\homb}{\hat{\underline\omega}}


\newcommand{\cimkd}{{\mycal C}^\flat}
\newcommand{\cimku}{{\mycal C}^\sharp}
\newcommand{\proj}{\textrm{pr}}
\newcommand{\Mclosed}{\bcM}%{\hskip10pt {\overline{\phantom{I}}\hskip-15pt{\mycal M}}}
\newcommand{\cg}{\,{\tilde {\!g}}}


\newcommand{\cM}{\mycal M}
\newcommand{\cN}{\mycal N}
\newcommand{\cE}{\mycal E}

\newcommand{\cAp}{{\mycal A}_{\mbox{\scriptsize phg}}}
\newcommand{\cApM}{\cAp(M)}
\newcommand{\stsg}{{\mathfrak g}}
\newcommand{\tf}{\widetilde f}
\newcommand{\complementaire}{\complement}
\newcommand{\remarks}{{\bf Remarks : }}


\newcommand{\mcB}{{\mycal B}}
%\newcommand{\cL}{{\mycal  L}}
\newcommand{\decal}{{\mycal D}}
\newcommand{\cC}{{\mycal C}}
\newcommand{\cB}{{\mycal B}}
\newcommand{\cG}{{\mycal G}}
\newcommand{\cCak}{{\cC}^\alpha_k}
\newcommand{\cU}{{\mycal  U}}
\newcommand{\backmg}{b} %background Riemannian metric
\newcommand{\Id}{\mbox{\rm Id}} %identity matrix
\newcommand{\sconst}{\mbox{\scriptsize\rm const}} %constants

\newcommand{\chnindex}[1]{\index{#1}}
\newcommand{\chindex}[1]{\index{#1}}
\newcommand{\bhindex}[1]{\chindex{black holes!#1}}


\newcommand{\tA}{\theta_\Al}
\newcommand{\Hau}{{\mathfrak H}}
\newcommand{\Ar}{\mbox{\rm Area}}
\newcommand{\Arm}{\mbox{\rm Area}_{S_2}}
\newcommand{\Al}{{\mathcal Al}}
\newcommand{\Hausone}{\Hau1}
\newcommand{\Htwohone}{\Hau^{2}}
\newcommand{\calS}{{\mathscr S}}
\newcommand{\BA}{B_\Al}
\newcommand{\Leb}{{\mathfrak L}}


\newcommand{\eqs}[2]{\eq{#1}-\eq{#2}}

\newcommand{\cW}{{\mycal W}}

\newcommand{\cA}{{\mycal A}}

%\def\ba{\begin{eqnarray}}
%\def\ea{\end{eqnarray}}
\def\nen{\nonumber}
%\def\half {{1\over 2}}
\def\Tau {{\mycal  T}}


\newcommand{\pihyp}{\partial_\infty\hyp}
\newcommand{\cMext}{{\mcM}_{\ext}}
\newcommand{\timkd}{{\mycal T}^\flat}
\newcommand{\timku}{{\mycal T}^\sharp}


\newcommand{\ro}{\rho}
\newcommand{\roo}{\bar{\ro}}


\newcommand{\les}{\lesssim}
\newcommand{\ges}{\gtrsim}
\def\piT{{\,^{(\T)}\pi}}
\def\Qr{\mbox{Qr}}
\def\flux{{\mbox{Flux}}}
\def\pa{\partial}
\def\onab{\overline{\nabla}}
\def\Db{{\bf {\bar {\,D}}}}
\def\Dh{{\bf {\hat {\,{D}}}}}
\def\laph{\hat{\Delta}}
\def\Null{\dot{\NN}^{-}}
\def\EE{{\mycal  E}}
\def\GG{{\mycal  G}}
\def\OO{{\mycal  O}}
\def\QQ{{\mycal  Q}}
\def\UU{{\mycal  U}}
\def\VV{{\mycal  V}}
\def\TT{{\mycal  T}}
\def\exp{\,\mbox{exp}}
\def\P{{\bf P}}
\def\vphi{\varphi}


\def \endprf{\hfill  {\vrule height6pt width6pt depth0pt}\medskip}
\def\emph#1{{\it #1}}
\def\textbf#1{{\bf #1}}
\newcommand{\Us}{\mbox{$U\mkern-13mu /$\,}}
\newcommand{\eql}{\eqlabel}
\def\medn{\medskip\noindent}

\def\Db{{^{(\Lb)}  D}}

\def\a{{\alpha}}
\def\b{{\beta}}
\def\ga{\gamma}
\def\Ga{\Gamma}
\def\eps{\epsilon}
\def\La{\Lambda}
\def\si{\sigma}
\def\Si{\Sigma}
\def\ro{\rho}
\def\th{\theta}
\def\ze{\zeta}
\def\nab{\nabla}
\def\varep{\varepsilon}

\def\aa{{\underline{\a}}}
\def\bb{{\underline{\b}}}
\def\bb{{\underline{\b}}}
\def\omb{{\underline{\om}}}
\def\Lb{{\underline{L}}}
\def\aaa{{\bold a}}

\newcommand{\trchb}{\tr \chib}
\newcommand{\chih}{\hat{\chi}}
\newcommand{\xib}{\underline{\xi}}
\newcommand{\etab}{\underline{\eta}}
\newcommand{\chibh}{\underline{\hat{\chi}}\,}
\def\chih{\hat{\chi}}
\def\trch{\mbox{tr}\chi}
\def\tr{\mbox{tr}}
\def\Tr{\mbox{Tr}}
\def\Xb{{\underline X}}
\def\Yb{{\underline Y}}


\def\rhoc{\check{\rho}}
\def\sic{\check{\si}}
\def\bboc{\check{\bb}}
\def\muc{\tilde{\mu}}

\def\AA{{\mycal  A}}
\def\BB{{\mycal  B}}
\def\MM{{\mycal  M}}
\def\NN{{\mycal  N}}
\def\II{{\mycal  I}}
\def\FF{{\mycal  F}}
\def\HH{{\mycal  H}}
\def\JJ{{\mycal  J}}
\def\KK{{\mycal  K}}
\def\Lie{{\mycal  L}}
\def\DD{{\mycal  D}}
\def\PP{{\mycal  P}}
\def\HH{{\mycal  H}}


\def\LL{{\mathcal L}}


\def\A{{\bf A}}
\def\B{{\bf B}}
\def\F{{\bf F}}
\def\I{{\bf I}}
\def\J{{\bf J}}
\def\M{{\bf M}}
\def\L{{\bf L}}
\def\O{{\bf O}}
\def\Q{{\bf Q}}
\def\R{{\mathbb R}}
\def\U{{\bf U}}
\def\S{{\bf S}}
\def\K{{\bf K}}
\def\g{{\bf g}}
\def\t{{\bf t}}
\def\u{{\bf u}}
\def\p{{\bf p}}
\def\LLb{{\bf \Lb}}

\def\Ab{\underline{A}}
\def\Eb{\underline{E}}
\def\Bb{\underline{B}}
\def\Hb{\underline{H}}
\def\Rb{\underline{R}}
\def\Vb{\underline{V}}
\def\AAA{{\Bbb A}}
\def\RRR{{\Bbb R}}
\def\MMM{{\Bbb M}}
\def\T{{\Bbb T}}
\def\To{\T}

\def\Aoc{\check{A}}
\def\Roc{\check{R}}
\def\nabb{\overline{\nab}}
\newcommand{\nabbb}{\mbox{$\nabla \mkern-13mu /$\,}}
\def\Ml{{\mycal  M}_{\ell}}
\def\intws{{\,\,\,\int_0^s \mkern-30mu \om}\,\,\,\,}
\def\expp{\mbox{exp}}

\def\B{{\bf B}}



\newcommand{\changedX}{K}

\newcommand{\hahyp}{\,\,\widehat{\!\!\hyp}}%

\def\lap{\Delta}
\def\pr{\partial}
\newcommand{\ddd}{\nab}

\def\c{\cdot}




\def\Da{{^{(A)}\hskip-.15 pc \D}}

\newcommand{\distb}{d_\backmg}
\newcommand{\hmcK}{\widehat \mcK}
\newcommand{\ptcx}[1]{\ptc{#1}}


\def\hot{\widehat{\otimes}}
\def\lot{\mbox{l.o.t.}}

\renewcommand{\div}{\mbox{div }}
\newcommand{\divv}{\mbox{div} }
\def\err{\mbox{Err}}
\newcommand{\lapp}{\mbox{$\bigtriangleup  \mkern-13mu / \,$}}

\newcommand{\piX}{\,^{(X)}\pi}
\def\diag{{\mbox{diag}}}
\def\Flux{\mbox{Flux}}
\def\En{\mbox{En}}
\def\ub{{\underline u}}
\def\dual{{\,^\star \mkern-3mu}}
\def\2{{\overline 2}}
\def\NI{\noindent}
\def\Cb{\underline C}

\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

